Sharing Frissons among Online Video Viewers: Exploring the Design of Affective Communication for Aesthetic Chills

On online video platforms, viewers often lack a channel to sense others' and express their affective state on the fly compared to co-located group-viewing. This study explored the design of complementary affective communication specifically for effortless, spontaneous sharing of frissons during video watching. Also known as aesthetic chills, frissons are instant psycho-physiological reactions like goosebumps and shivers to arousing stimuli. We proposed an approach that unobtrusively detects viewers' frissons using skin electrodermal activity sensors and presents the aggregated data alongside online videos. Following a design process of brainstorming, focus group interview (N=7), and design iterations, we proposed three different designs to encode viewers' frisson experiences, namely, ambient light, icon, and vibration. A mixed-methods within-subject study (N=48) suggested that our approach offers a non-intrusive and efficient way to share viewers' frisson moments, increases the social presence of others as if watching together, and can create affective contagion among viewers.

==> sections/introduction-old.tex <==
\section{Introduction}

Affective communication is a prevalent and important activity in people's everyday social interactions.
Here, affects refer to
``the states of organism that have both organic and psychological components''~\cite{schererNatureFunctionEmotion1984}.
Affective communication refers to perceive others' and share our own affects~\cite{garridoAudienceEngagementCommunity2020},
and affective experience is the personal experience of such affects~\cite{kootsInfluenceWeatherAffective2011}.
Hence, affects are a generic concept that includes but is not limited to emotions,
which are only a subset of psychological processes~\cite{schweiger-galloProspectsDilemmasEmotion2010}.
Specifically when people watch videos, performances, etc., together,
several affects are triggered
e.g., excitement~\cite{heFrissonWavesExploring2022},
cheerfulness~\cite{wangSensingLiveAudience2014},
aesthetic chills (having goosebumps)~\cite{neidlingerAWElectricThatGave2017,heFrissonWavesExploring2022}.
The communication of such affects
often leads to a contagious effect~\cite{wetherellAffectEmotionNew2012,guoPreliminaryStudyEmotional2020},
and an enhanced individual affective experience~\cite{garridoAudienceEngagementCommunity2020}.
Furthermore, it can create stronger bonding
and a sense of belonging among the audience community~\cite{garridoAudienceEngagementCommunity2020,hilvert-bruceSocialMotivationsLivestreaming2018,pittsWhatMakesAudience2005,wulfWatchingPlayersExploration2020}.
Such an impact of affective communication among the audience is commonly identified in various events like
musical concerts~\cite{garridoAudienceEngagementCommunity2020,pittsWhatMakesAudience2005},
live-streaming~\cite{hamiltonStreamingTwitchFostering2014,hilvert-bruceSocialMotivationsLivestreaming2018,wulfWatchingPlayersExploration2020},
and sports events~\cite{vatavuAudienceSilhouettesPeripheral2015}.

Apart from the aforementioned events,
another context where affective communication is needed by the audience is
when people watch videos online~\cite{centieiroIfYouCan2014}.
But for regular online video platforms like YouTube,
viewer activities are usually conducted remotely and asynchronously:
they watch the same video at different places and different time.
Therefore, it is hard to communicate and know other viewers' states when watching the video,
especially others' reactions to specific moments of the video.
In attempts to fulfil such a need, several designs are presented for online video platforms
--- often generic but allow affective communication to some extent.
The most traditional comment area allows post-hoc textual discussion in a threaded manner.
Due to its separation from the video timeline,
it is cumbersome to convey viewers' instant change of feelings with the content.
Recently, time-synced comments also appear,
often in a scrolling comment area
or overlaid on top of the video content (a.k.a.\@ \emph{Danmaku})~\cite{maVideobasedEvanescentAnonymous2017}.
But it requires attention and cognitive loads to comprehend textual comments whilst watching the video.
Thus, it can distract users' attention and interrupt the experiences.
For Danmaku, it will also obscure the video content and diverge users' attention~\cite{maVideobasedEvanescentAnonymous2017,chenWatchingMovieAlone2017}
% This is especially common at critical moments of the video when the audience's emotions are largely aroused.
And it can also have a delay behind the actual moments to comment due to users' typing.
For either type of comments,
it requires viewers to actively engage in the writing,
interrupting the watching experience as well as demanding extra cognitive load.
There are also some visualizations of user behaviors.
On YouTube, the “popular segments” plot above the progress bar indicates the most-loved parts by the times each moment is played.
On a popular Chinese online video platform, Bilibili, the Danmaku count distribution is plotted above the progress bar.
Both designs indirectly reveal viewers' affects at specific moments via behavioral data,
but such indication is not always accurate,
as viewers may replay or comment a segment due to other reasons.

Therefore,
although text-based viewer interactions are expressive and versatile,
a lightweight system can be designed as an effective supplement
to specifically foster affective communication among the audience.
It can draw inspirations from user behavior feedback designs mentioned above,
so that it offers unobtrusive input and display
and conveys viewers' instant changes of feelings at the corresponding moments in the video.

To design an effective and unobtrusive channel for affective communication among online video viewers,
one desirable tool is biosignals.
Biosignals are the signals or measurements generated by the human body that indicate the bodily functions and activities, such as heart rate, respiration rate, skin conductance (EDA, a.k.a.\@ GSR), and muscle activities (EMG).
They are directly related to the individual's affects~\cite{betellaInferenceHumanAffective2014},
and the audience often experience variations in biosignals with their affects
during the watching experience~\cite{tschacherPhysiologicalSynchronyAudiences2023,heFrissonWavesExploring2022}.
Also, they can be sensed non-intrusively by wearable sensors.
Thus, it can be used as a medium of affective communication to create a more engaging viewer experience on online video platforms,
while maintaining users' main attention to the video content.

In this paper,
we would like to explore the potential of biosignal sensing and feedback on online video platforms
in terms of affective communication and viewers' individual affective experience.
More formally,
this paper aims to answer the following research questions (RQ) through the design and evaluation of a biosignal sensing and feedback system.
\begin{enumerate}[RQ1]
    \item Will sensing and feedback of viewers' biosignals facilitate their affective communication on online video platforms?
    \item Will sensing and feedback of viewers' biosignals improve their individual affective experience on online video platforms?
    \item What are the design implications of viewers' biosignal feedback on online video platforms to provide the best user experience?
\end{enumerate}

Our research...
\begin{quote}
\fbox{\parbox{\linewidth}{Introduce the work after I finish the latter parts}}
\end{quote}

The key contribution of this research is as follow:
\begin{itemize}
    \item A system for online video platforms to collect viewers' biosignals unobtrusively and provide feedback with minimal cognitive loads.
    \item The evaluation of the system and several design considerations for future work of asynchronous affective communication systems using biosignals.
\end{itemize}
